Sequential Printed MLP Circuits for Super TinyML Multi-Sensory Applications

Super-TinyML aims to optimize machine learning models for deployment on ultra-low-power application domains such as wearable technologies and implants. Such domains also require conformality, flexibility, and non-toxicity which traditional silicon-based systems cannot fulfill. Printed Electronics (PE) offers not only these characteristics, but also cost-effective and on-demand fabrication. However, Neural Networks (NN) with hundreds of features -- often necessary for target applications -- have not been feasible in PE because of its restrictions such as limited device count due to its large feature sizes. In contrast to the state of the art using fully parallel architectures and limited to smaller classifiers, in this work we implement a super-TinyML architecture for bespoke (application-specific) NNs that surpasses the previous limits of state of the art and enables NNs with large number of parameters. With the introduction of super-TinyML into PE technology, we address the area and power limitations through resource sharing with multi-cycle operation and neuron approximation. This enables, for the first time, the implementation of NNs with up to $35.9\times$ more features and $65.4\times$ more coefficients than the state of the art solutions.

==> tables/oldtab_feataccarea.tex <==
\begin{table}
  \caption{\red{Evaluation of Features before and after RFP, Accuracy and Area}}
  \label{tab:feataccarea}
  % \renewcommand{\arraystretch}{0.9}
  \vspace{-1ex}

  \begin{tabular}{p{1cm} | p{0.8cm} p{1.3cm} | p{1.2cm} p{2.2cm}}
    % \centering
    \toprule
    Dataset & Feat. & Feat. (post RFP) & Accuracy & Area ($cm^2$) (Our Multi-cycle Seq.)\\
    \midrule
    SPECTF & 44 & 38 & 87.50 & 12.84 \\
    Arr. & 274 & 155 & 61.76 & 24.27 \\
    Gas S. & 128 & 118 & 90.65 & 24.93 \\
    Epi. & 178 & 169 & 93.45 & 25.18 \\
    Act. & 533 & 276 & 80.50 & 26.65 \\
    Par. & 753 & 620 & 85.02 & 23.58 \\
    HAR & 561 & 557 & 96.90 & 70.60 \\
    \bottomrule
\end{tabular}
\vspace{-1ex}
\end{table}

==> tables/tab_gains5.tex <==

\begin{table}
  \caption{Gains of Neuron Approximation with 5\% Accuracy Drop Tolerance w.r.t. DATE2023\cite{Kokkinis:DATE2023}+Feature Sel.}
  \label{tab:gains5}
  % \renewcommand{\arraystretch}{0.9}
  \begin{tabular}{l|ccc}
    % \centering
    \toprule
    Dataset & Area  & Power \\
      &  gains &  gains \\
    \midrule
    SPECTF & 2.9$\times$ & 1.5$\times$ \\
    Gas Sensor & 8.6$\times$ & 5.2$\times$ \\
    Epileptic Seizure & 12$\times$ & 6.7$\times$ \\
    Arrhythmia & 6.5$\times$ & 4.0$\times$\\
    HAR & 23$\times$ & 15$\times$ \\
    Parkinsons & 34$\times$ & 23$\times$ \\
    \midrule
    Average & \textbf{14}$\times$ & \textbf{8.7}$\times$\\
    \bottomrule
\end{tabular}
\end{table}

%gains of DATE+feature sel. and 5% acc drop.

==> tables/tab_parameters.tex <==
\begin{table}
  \caption{Applications for printed MLPs}
  \label{tab:parameters}
  % \renewcommand{\arraystretch}{0.9}

  \begin{tabular}{ccl}
    % \centering
    \toprule
    Application & Sensors & Coefficients\\
    \midrule
    Breast Cancer & 10 & 36 \\
    Cardio & 21 & 72 \\
    Pendigits & 16 & 130  \\
    RedWine & 11 & 34 \\
    \midrule
    SPECTF & 44 & 322  \\
    Gas Sensor & 128 & 1474 \\
    Epileptic Seizure & 178 & 1980 \\
    Arrhythmia & 274 & 1450 \\
    HAR & 561 & 8505 \\
    Parkinsons & 753 & 6040 \\
    \bottomrule
\end{tabular}
\vspace{0.5ex}
\end{table}
